Constraint Solving with Deep Learning for Symbolic Execution

Symbolic execution is a powerful systematic software analysis technique, but suffers from the high cost of constraint solving, which is the key supporting technology that affects the effectiveness of symbolic execution. Techniques like Green and GreenTrie reuse constraint solutions to speed up constraint solving for symbolic execution; however, these reuse techniques require syntactic/semantic equivalence or implication relationship between constraints. This paper introduces DeepSover, a novel approach to constraint solving with deep learning for symbolic execution. Our key insight is to utilize the collective knowledge of a set of constraint solutions to train a deep neural network, which is then used to classify path conditions for their satisfiability during symbolic execution. Experimental evaluation shows DeepSolver is highly accurate in classifying path conditions, is more efficient than state-of-the-art constraint solving and constraint solution reuse techniques, and can well support symbolic execution tasks.

==> Sections/06Discussion.tex <==
%************************************************
\section{Discussion} \label{discussion}
%************************************************

% In this section, we have some further discussion on our technique,
% focusing on the two factors that may have impact on the performance of
% the approach.

\subsection{Matrix Size} \label{matrixsize} 

As introduced in Section~\ref{DeepSolver}, there are three major
factors of a path condition that are used to decide the size of
matrix: number of different symbolic variables, number of 
constraints, and the highest degree of the path condition. In our
design, a path condition of a smaller dimension can be easily expanded
to a path condition of a larger dimension by setting the corresponding
items of the matrix with value 0 (``$padding$''). Padding enables a
high flexibility on the selection of the size of matrix, and a less
number of matrix we use means a less number of DNNs we need to
train. Also, padding increases the applicability of our approach, for
it is possible for us to set up a reasonably large matrix size in
order to support complex path conditions.

However, we would like to argue that padding can also lead to an
unwanted side effect in training. More specifically, a large number of
paddings in training data may lead to over-fitting problem. Consider a
simple example where we setup a unified matrix size of linear path
condition with 2 variables and 20 constraints, and assume all
the path conditions we used for training are with exactly 2 symbolic
variables and only 15 constraints. In this case, each path
condition needs 5 extra padding rows, where all the items are set to
0. If we use these data to train a DNN, it is highly possible that the
weight of the padding rows are very low for the data lack
diversity. Thus, even though the DNN can accept a real path condition
with 2 variables and 20 constraints, the classification is in
fact not considering the last 5 rows equally important than the first
15 rows. % which is obviously against common sense of mathematics.
Also, a larger matrix means there are more data that need to go
through the DNN, which will have a negative impact on the efficiency
of our technique.

Ideally, a DNN should be trained and used to classify path conditions
that do not need any padding, and the less padding we use, the more
persuasive and accurate the classification can be. However, it also
requires the training data set to be further
distinguished. Unfortunately, due to the nature of software and
limitation of constraint solvers, collecting enough data for highly
complex path conditions can be challenging. In our current
implementation, we set up multiple matrix sizes based on the number of
constraints. However, we cannot further bring it down to set up
matrix based on the number of symbolic variables or nonlinear path
conditions, for we cannot gather enough training data for the DNNs we
need. Although the evaluation results still show a very high accuracy,
we would like to argue that a further improvement to use more refined
matrix should be done if possible. Meanwhile, with a more clever
transforming, we can potentially minimize the negative impact of
padding and still take advantage of the flexibility it brings us. For
instance, we can shuffle the actual data and padding data in the
matrix with a certain rule so that the padding rows are not always at
the end of a matrix. In this way, diversity of training data is
increased without adding more records to the data set.

\subsection{DNN Structure} \label{nnstructure} 

The structure of a DNN is an important factor that has much to do
with the efficiency of our approach. In general, larger network means
the input data needs to go through a greater number of neurons and a
more complex computation to reach the classification result, which
eventually leads to a higher time cost.

How to setup the hidden layers of a DNN is a hot topic in research. In
our implementation and evaluation, we made a conservative assumption
on the structure and started with a relatively large DNN
structure. Our insight is a larger DNN is more competent to the
problem. The evaluation results showed that our initial $10 \times 10$
structure is getting an almost perfect accuracy. But to our surprise,
the performance did not get worse when we shrinked the structure to
$5 \times 5$. This shows that there is still a space to optimize the
structure to further reduce the time cost while maintaining a high
accuracy. Moreover, different data matrix sizes (as we discussed in
Section \ref{matrixsize}) may have their own best DNN structure, which
is a very interesting topic to explore for our future work.

% \subsection{Efficiency of DNN} \label{efficiency}
% As we discussed, the efficiency of our technique purely depends on the matrix size, the DNN structure, and number of path condition generated. Evaluation result shows an expected result that for the same subject, where the matrix size ad number of path condition is fixed, the time cost is stable and only related to the structure of a DNN. In other words, our technique takes no impact from the complexity of path conditions, which is essential for both conventional symbolic execution and Green framework. On one hand, it means that our technique can classify complex path conditions which a traditional solver needs a lot of time or even is not capable to solve. On the other hand, for simple path conditions that can be easily solved or reused, using a DNN may actually hurt the performance, as the scaling is almost impossible once the DNNs are finalized and applied.

% Apart from setting up a diversity of DNNs which we discussed above, another potential solution is to construct a hybrid framework that applies traditional solver, conventional constraint solution reusing approach, and DNN at the same time. Theoretically, a straight reuse of former path condition solving results should be the fastest, while constraint solving and DNN compete based on the complexity of the incoming path condition. Thus, all three solutions can be set to run at the same time, and once the satisfiablity result is generated by either one of them, other two approaches will be stopped, and result can be insert into the database for future reusing or training purposes.

% % Actually I am not quite sure about if we should mention this next paragraph, but I decide to put it here anyway for the sake of our future work.
% Meanwhile, traditional constraint solvers can also be used to confirm the DNN classification result. Despite the high accuracy reported for some data sets by the engine, an 100\% accurate DNN on any future data set is almost impossible to get. Thus, for critical paths that are more interesting, users can choose to randomly double-check the classification result of DNN with a conventional constraint solver.

% \subsection{Limitations} \label{limitation} 

% One limitation of our technique is that unlike traditional constraint
% solvers, which can provide a set of actual values to satisfy or
% violate a path condition, a DNN can only classify whether a path
% condition is satisfiable or not. In other words, in the current state
% of development, our DNN cannot fully replace a constraint solver, and
% can only be applied while the solution in terms of the values of
% symbolic input variables is not necessary. DNNs are able to quickly
% detect infeasible paths, but not yet capable to generate test inputs
% for a feasible path.  For this reason, we need to choose the
% application scenario of our technique before a reliable DNN can fully
% replace constraint solvers. For example, since test inputs are
% generally needed only for complete paths, we can potentially combine
% our approach with regular constraint solving, while regular constraint
% solving is only used when a complete path is explored.



==> Sections/07Threat.tex <==
%************************************************
\section{Threat to Validity} \label{threat}
%************************************************
There are some threats to validity associated to the results we presented.

\subsection{External Validity} \label{external}
In terms of external validity, our results might not generalize to other subjects. Our study was performed over popular artifacts used among studies of symbolic execution techniques, and we picked out the subjects and versions that are suitable for our technique including data collection, training and evaluation purposes. To mitigate this threat we trained and selected multiple models, and carefully selected the results that can be potentially generalized, but it should be noticed that in deep learning studies, it is not uncommon that a well-trained model cannot be used as a universal solution to similar but different artifacts.

Another external threat to validity lies in records in the database. Since infeasible paths is considered as a programming error in most common cases, it is natural that the number of satisfiable PCs far exceeds the number of unsatisfiable PCs. As a result, unlike conventional deep learning techniques, it is very difficult for us to collect a balanced database for training. However, after carefully examine the result, we find that our DNNs are still able to classify unsatisfiable PCs correctly with a low data-loss, which means the impact of such threat is minimized in our approach.

\subsection{Internal Threats} \label{internal}
In terms of internal validity, although we have carefully checked our implementation, it is possible that there are errors we did not notice. There are also potential threats related to correctness of the foundation techniques and frameworks we used, including Keras, Tensorflow and Symbolic Pathfinder. To mitigate this threat, we treat them as black-box models to ensure that we only made the necessary change to the original SPF implementation.

Over-fitting is a common problem when training a DNN. In our evaluation, we apply multiple approaches to avoid this problem and the results show no evidence of over-fitting happening in our training process. Yet, we believe it is important to list it as one of the threats to validity to show we attach great importance to this problem.


==> Sections/Overfitting.tex <==
\subsection{Overfitting} \label{overfitting}
\begin{table}[!htb]
\caption[NNAD]{Neural Network Accuracy and Data-loss}
\begin{center}
\begin{tabular}{ | c || c | c | c | }
\hline
Matrix Size	& 	\# of Data	& Accuracy	& Data-loss \\ \hline \hline
$22 \times 11$	&	5,136		& 100\%	& 0.003 	\\ \hline
$22 \times 12$	&	1,005		& 99.5\%	& 0.017 	\\ \hline
$22 \times 13$	&	18,519		& 98.8\%	& 0.012 	\\ \hline
$22 \times 14$	&	33,251		& 99.2\%	& 0.013 	\\ \hline
$22 \times 15$	&	58,965		& 99.8\%	& 0.006 	\\ \hline
$22 \times 16$	&	82,773		& 98.6\%	& 0.002 	\\ \hline
$22 \times 17$	&	108,174		& 98.2\%	& 0.009	\\ \hline
$22 \times 18$	&	134,862	& 100\%	& 0.006 	\\ \hline
$22 \times 19$	&	151,173		& 100\%	& 0.004 	\\ \hline
$22 \times 20$	&	138,894	& 100\%	& 0		 	\\ \hline
$22 \times 21$	&	133,395	& 100\%	& 0.001 	\\ \hline
$22 \times 22$	&	117,265		& 100\%	& 0.001 	\\ \hline
$22 \times 23$	&	98,307		& 100\%	& 0		 	\\ \hline
$22 \times 24$	&	74,705		& 100\%	& 0	 		\\ \hline
$22 \times 25$	&	49,498		& 100\%	& 0		 	\\ \hline
$22 \times 26$	&	33,051		& 100\%	& 0	 		\\ \hline
$22 \times 27$	&	19,182		& 100\%	& 0.004 	\\ \hline
$22 \times 28$	&	7,410		& 100\%	& 0		 	\\ \hline	
\end{tabular}
\end{center}
\label{tab:NNAD}
\end{table}

Table \ref{tab:EvaResult2} shows that the accuracy of our
classification is as high as over 98\% which is good in most cases. Yet,
since we are using deep learning, we need to consider the possibility
of over-fitting. An over-fitting happens when the model is overly
refined to the training data which makes the DNN capable of
classifying some data extremely accurately, while the performance
drops dramatically on different data sets. As a result, it makes the
DNN not reliable in real applications. Generally speaking, as long as
the performance (including accuracy and data-loss) on training set and
evaluation subjects are close enough, the doubt of over-fitting can be
eliminated. However, since the accuracy of our DNN is extremely high
and we are using an overall performance from multiple DNNs, we
consider it important to have a deeper look into this problem.

To further investigate the possibility of over-fitting, we checked all
the DNNs separately. Since Table \ref{tab:EvaResult2} already shows the
accuracy on the chosen subjects, in order to reinforce the data, we
generate more path conditions collected from mutants of these subjects
and check the classification accuracy of each DNN. Table
\ref{tab:NNAD} shows the accuracy and data-loss for all the DNNs we trained. While accuracy shows the correctness of the final classification result, data-loss shows the errors between this result and the actual label. In other words, a smaller data-loss means that the predicted results compromised less to be classified correctly, and thus the accuracy data is more persuasive.

%\ref{tab:NNAD} shows the accuracy (correctness of the final
%classification result) and data-loss (difference between the generated
%results and the classification value) for all the DNNs we trained. % We
% first run the subjects with {Green} to generate databases of path
% conditions, and then apply them to the DNNs with Keras to collect the
% accuracy and data-loss.

As we can see in Table \ref{tab:NNAD}, for all the 18 DNNs we trained,
the accuracy is very high (above $98.2\%$) while the data-loss is very
low (less than $0.02$, while in most cases it is very close to $0$)
with the new data set. Meanwhile, we would like to mention that we
have used different approaches to avoid over-fitting when we were
training the DNNs, including purifying and shuffling the data,
changing the ratio of training/testing data, using different DNN
structures and applying k-fold validation technique. In the whole
process, we did not observe any large change in accuracy and
data-loss. Thus, we believe it is safe to claim that our approach in
classifying path conditions for satisfiability is effective, and there
is no trace of over-fitting problem.

